Multi-Criteria Radio Spectrum Sharing With Subspace-Based Pareto Tracing

Radio spectrum is a high-demand finite resource. To meet growing demands of data throughput for forthcoming and deployed wireless networks, new wireless technologies must operate in shared spectrum over unlicensed bands (coexist). As an example application, we consider a model of Long-Term Evolution (LTE) License-Assisted Access (LAA) with incumbent IEEE 802.11 wireless-fidelity (Wi-Fi) systems in a coexistence scenario. This scenario considers multiple LAA and Wi-Fi links sharing an unlicensed band; however, a multitude of other scenarios could be applicable to our general approach. We aim to improve coexistence by maximizing the key performance indicators (KPIs) of two networks simultaneously via dimension reduction and multi-criteria optimization. These KPIs are network throughputs as a function of medium access control (MAC) protocols and physical layer parameters. We perform an exploratory analysis of coexistence behavior by approximating active subspaces to identify low-dimensional structure in the optimization criteria, i.e., few linear combinations of parameters for simultaneously maximizing LAA and Wi-Fi throughputs. We take advantage of an aggregate low-dimensional subspace parametrized by approximate active subspaces of both throughputs to regularize a multi-criteria optimization. Additionally, a choice of two-dimensional subspace enables visualizations augmenting interpretability and explainability of the results. The visualizations and approximations suggest a predominantly convex set of KPIs over active coordinates leading to a regularized manifold of approximately Pareto optimal solutions. Subsequent geodesics lead to continuous traces through parameter space constituting non-dominated solutions in contrast to random grid search.

==> Sys_Model.tex <==
We consider a downlink coexistence scenario where two mobile network operators (MNOs) operate over the same shared unlicensed industrial, scientific, and medical (ISM) radio band. We are primarily focused on the operation of cellular base stations in the unlicensed bands. However, LTE base stations may have permission to utilize a licensed band as well. We assume the MNOs use time sharing to simultaneously operate in the unlicensed band and we aim to analyze competing trade-offs in throughputs of the Wi-Fi and LTE-LAA systems. A network throughput is a function of both MAC and PHY layer parameters. In this section, we introduce the parameters defining the network topology, MAC
layer protocols, the PHY layer, and briefly discuss the relation of these variables to network throughput.

\subsection{Network Topology}
We consider a coexistence scenario in which the LTE-LAA network consists of $L$ Evolved Node B (eNodeBs) indexed by the set $\mathcal{L}$, $i \in \mathcal{L} = \lbrace 1,2,\dots,L\rbrace$, while the Wi-Fi network is composed of
$W$ access points (APs) indexed by the set $\mathcal{W}$, $j \in \mathcal{W} = \lbrace 1,2,\dots,W \rbrace$. Note that our proposed subspace-based Pareto tracing approach could be applied to many types of communication systems (or alternative applications), but LTE is used here as an example. The eNodeBs and APs are randomly distributed over a
particular area while LAA user equipment (UEs) and Wi-Fi clients/stations (STAs) are respectively distributed around each eNodeB and AP independently and uniformly. Each transmission node serves one single antenna UEs/STAs. %We assume any transmission
% node \deleted[id=ZG]{indexed by $\mathcal{L}$ or $\mathcal{W}$ transmits with $P_{k}$, $k \in \{\mathcal{L}, \mathcal{W}\}$, and the} and user association is based on the received power. 
We assume \textit{(i)} both Wi-Fi and LAA are in the saturated traffic condition, i.e., at least one packet is waiting to be sent, \textit{(ii)} there are neither hidden nodes nor false alarm/miss detection problems in the network\footnote{We assume perfect spectrum sensing in both systems. The impact of imperfect sensing is beyond the scope of this paper and investigating the effect of sensing errors is an important topic for future work.}, \textit{(iii)} the channel knowledge is ideal, so the only source of unsuccessful transmission is collision, \textit{(iv)} a successful transmission happens if only one link transmits at a time, i.e.,
exclusive channel access (ECA) model is considered, and \textit{(v)}  each link is subject to Rayleigh fading and Log-normal shadowing.

\subsection{MAC Layer Protocols}
The medium access key feature in both Wi-Fi and LAA involves the station accessing the medium to sense the channel by performing clear channel assessment prior to transmitting. The station only transmits if the medium is determined to be idle. Otherwise, the transmitting station refrains from transmitting data until it senses the channel is available. Although LAA and Wi-Fi technologies follow similar channel access procedures, they utilize different carrier sense schemes, different channel sensing threshold levels, and different channel contention parameters, leading to different unlicensed channel access probabilities and thus, different throughputs.

%Here, we will briefly describe the network throughput of both systems, a quantity that will be used in analyzing competing trade-offs in throughputs of the Wi-Fi and LTE-LAA systems later.
Conforming with the analytical model in \cite{Bianchi-2000}, the probability of either network transmitting a packet in a randomly chosen time slot can be expressed as 
\begin{multline} \label{Eqn_1}
p_{k}(c_{k}; \omega_{k}, \mu_{k}) =\\ \frac{2(1 - 2 c_{k})}{(1-2c_{k})(1 + \omega_{k}) + c_{k}\omega_{k}(1-(2c_{k})^{\mu_{k}})}, 
\end{multline}
where $k$ is representative of an index from either $\mathcal{L}$ or $\mathcal{W}$, $c_{k}$ denotes the probability of collision experienced by the $k$-th transmission node, and $\omega_{k}$ and $\mu_{k}$ indicate the minimum contention window size and the maximum back-off stage, respectively, of the $k$-th transmission node on the unlicensed channel. 

\begin{table*}[t]
\captionsetup{font=footnotesize}
 \caption{Probabilities of time slot allocations}\label{tbl:probs}
 \begin{threeparttable}
 \centering
 \scalebox{0.98}{
 \scriptsize
  \begin{tabular}{c|p{8cm} |l}
    \hline
    Probability & Description & Expression \\ \hline
    %\rowcolor{LightCyan}
     $(\boldsymbol{p}_{\mathcal{T}})_1$ & Probability unlicensed band is idle & $\det\left( \text{diag}\left(\boldsymbol{p}_{\mathcal{W}}^{\complement}\right)\right) \det\left(\text{diag}\left(\boldsymbol{p}_{\mathcal{L}}^{\complement}\right)\right)$\\[0.1cm] %\hline
      %\rowcolor{LightCyan}
    $(\boldsymbol{p}_{\mathcal{T}})_2$ & Overall probability of successful Wi-Fi transmission on the unlicensed band & $\boldsymbol{1}_{\mathcal{W}}^\transpose\boldsymbol{s}_{\mathcal{W}} = \boldsymbol{p}_{\mathcal{W}}^{\transpose}\boldsymbol{c}_{\mathcal{W}}^{\complement}$\\[0.1cm] %\hline
      %\rowcolor{LightCyan}
      $(\boldsymbol{p}_{\mathcal{T}})_3$ & Overall probability of successful LAA transmission on the unlicensed band & $\boldsymbol{1}_{\mathcal{L}}^\transpose\boldsymbol{s}_{\mathcal{L}} = \boldsymbol{p}_{\mathcal{L}}^{\transpose}\boldsymbol{c}_{\mathcal{L}}^{\complement}$\\[0.1cm] %\hline
      %\rowcolor{LightCyan}
      $(\boldsymbol{p}_{\mathcal{T}})_4$ & Probability of collision among the Wi-Fi transmissions & $\det\left( \text{diag}(\boldsymbol{p}_{\mathcal{L}}^{\complement})\right)\left[1- \det\left( \text{diag}(\boldsymbol{p}_{\mathcal{W}}^{\complement})\right) -  \boldsymbol{\iota}_{\mathcal{W}}^{\transpose}\boldsymbol{p}_{\mathcal{W}}\right]$\\[0.1cm] %\hline
      %\rowcolor{LightCyan}
      $(\boldsymbol{p}_{\mathcal{T}})_5$ & Probability of collision among the LAA transmissions & $\det\left( \text{diag}(\boldsymbol{p}_{\mathcal{W}}^{\complement})\right)\left[1- \det\left( \text{diag}(\boldsymbol{p}_{\mathcal{L}}^{\complement})\right) - \boldsymbol{\iota}_{\mathcal{L}}^{\transpose}\boldsymbol{p}_{\mathcal{L}}\right]$\\[0.1cm] %\hline
      %\rowcolor{LightCyan}
      $(\boldsymbol{p}_{\mathcal{T}})_6$ & Probability of collision among Wi-Fi \& LAA transmissions &$\left[1 - \det\left( \text{diag}(\boldsymbol{p}_{\mathcal{L}}^{\complement})\right)\right]\left[1 - \det\left( \text{diag}(\boldsymbol{p}_{\mathcal{W}}^{\complement})\right)\right]$ %\hline
      %\rowcolor{LightCyan}
    \end{tabular}}
   \end{threeparttable}
\end{table*}
\normalsize

To simplify notation, we aggregate the stationary transmission probability model \eqref{Eqn_1} into entries of a vector-valued function $\boldsymbol{p}$. With this notation, the stationary transmission probability of AP $j \in \mathcal{W}$ is written as, $(\boldsymbol{p})_j:(c_{j}, \omega_{j}, \mu_{j})\mapsto p_{j}(c_{j}; \omega_{j}, \mu_{j})$ and $\boldsymbol{p}_{\mathcal{W}} \overset{\Delta}{=} \boldsymbol{p}(\boldsymbol{c}_{\mathcal{W}}; \boldsymbol{\omega}_{\mathcal{W}}, \boldsymbol{\mu}_{\mathcal{W}})$ represent the set of probabilities and parameters for all Wi-Fi APs, $\boldsymbol{p}_{\mathcal{W}}, \boldsymbol{c}_{\mathcal{W}},\boldsymbol{\omega}_{\mathcal{W}},\boldsymbol{\mu}_{\mathcal{W}} \in \mathbb{R}^{W}$. Similarly, for the LAA eNodeB's, we assign $\boldsymbol{p}_{\mathcal{L}} \overset{\Delta}{=} \boldsymbol{p}(\boldsymbol{c}_{\mathcal{L}}; \boldsymbol{\omega}_{\mathcal{L}}, \boldsymbol{\mu}_{\mathcal{L}})$ such that $\boldsymbol{p}_{\mathcal{L}}, \boldsymbol{c}_{\mathcal{L}},\boldsymbol{\omega}_{\mathcal{L}},\boldsymbol{\mu}_{\mathcal{L}} \in \mathbb{R}^{L}$.

Note, for brevity, we drop the explicit dependencies, $p_{j}(c_{j}; \omega_{j}, \mu_{j})$, and supplement with an index-set subscript, $\boldsymbol{p}_{\mathcal{W}}$, to indicate the length of the vector in addition to the network association. With this notation, we can write the LAA and Wi-Fi overall probability of transmission as $\prod_{i\in \mathcal{L}}(1 - \boldsymbol{e}_i^\transpose\boldsymbol{p}_{\mathcal{L}})$ and $\prod_{j\in \mathcal{W}}(1 - \boldsymbol{e}_j^\transpose\boldsymbol{p}_{\mathcal{W}})$, respectively, where $\boldsymbol{e}_i$ (resp. $\boldsymbol{e}_j$) is the $i$-th (resp. $j$-th) column of the appropriately sized identity matrix. In a complementary fashion, the collision probability of the transmitting Wi-Fi AP $j$ and LAA eNodeB $i$ on a shared unlicensed band are expressed as entries $(\boldsymbol{c}_{\mathcal{W}})_{j}$ and $(\boldsymbol{c}_{\mathcal{L}})_{i}$, respectively, in the vectors
\begin{align} \label{eq:Wifi_collision}
    \boldsymbol{c}_{\mathcal{W}} = \boldsymbol{1}_{\mathcal{W}} -\boldsymbol{\iota}_{\mathcal{W}} \prod_{i\in \mathcal{L}}(1 - \boldsymbol{e}_i^{\transpose}\boldsymbol{p}_{\mathcal{L}}),
\end{align}
and
\begin{align} \label{eq:LAA_collision}
\boldsymbol{c}_{\mathcal{L}} = \boldsymbol{1}_{\mathcal{L}} - \boldsymbol{\iota}_{\mathcal{L}} \prod_{j \in \mathcal{W}}(1-\boldsymbol{e}_j^{\transpose}\boldsymbol{p}_{\mathcal{W}}),
\end{align}
where the intersection of complementary transmission events is denoted
\begin{align}\nonumber
(\boldsymbol{\iota}_{\mathcal{K}})_k \overset{\Delta}{=} \frac{1}{1 - \boldsymbol{e}_{k}^{\transpose}\boldsymbol{p}_{\mathcal{K}}}\prod_{q\in \mathcal{K}}(1 - \boldsymbol{e}_q^\transpose\boldsymbol{p}_{\mathcal{K}});
\end{align}
where $\mathcal{K}$ is a placeholder for either index set $\mathcal{W}$ or $\mathcal{L}$. Notice, \eqref{eq:Wifi_collision} and \eqref{eq:LAA_collision} are vector-valued maps acting on both $\boldsymbol{p}_{\mathcal{L}}$ and $ \boldsymbol{p}_{\mathcal{W}}$ given parameters $\boldsymbol{\omega}_{\mathcal{W}}, \boldsymbol{\mu}_{\mathcal{W}},\boldsymbol{\omega}_{\mathcal{L}}, \boldsymbol{\mu}_{\mathcal{L}}$. Precisely, equations \eqref{eq:Wifi_collision} and \eqref{eq:LAA_collision} represent a coupling of the vector-valued maps such that $\boldsymbol{c}_{\mathcal{W}} \overset{\Delta}{=} \boldsymbol{c}(\boldsymbol{p}_{\mathcal{W}}, \boldsymbol{p}_{\mathcal{L}}; \boldsymbol{\omega}_{\mathcal{W}}, \boldsymbol{\mu}_{\mathcal{W}},\boldsymbol{\omega}_{\mathcal{L}}, \boldsymbol{\mu}_{\mathcal{L}})$ where the first input  $\boldsymbol{p}_{\mathcal{W}}$ corresponds to the label, $\mathcal{W}$, and the form of $\boldsymbol{c}$ is inferred from \eqref{eq:Wifi_collision} or \eqref{eq:LAA_collision}---similarly for the LAA network, $\boldsymbol{c}_{\mathcal{L}} \overset{\Delta}{=} \boldsymbol{c}(\boldsymbol{p}_{\mathcal{L}}, \boldsymbol{p}_{\mathcal{W}}; \boldsymbol{\omega}_{\mathcal{W}}, \boldsymbol{\mu}_{\mathcal{W}},\boldsymbol{\omega}_{\mathcal{L}}, \boldsymbol{\mu}_{\mathcal{L}})$.

The probability of a successful transmission for the Wi-Fi AP $j$ and the LAA eNodeB $i$ on the unlicensed band are calculated as the entries $( \boldsymbol{s}_{\mathcal{W}})_{j}$ and $(\boldsymbol{s}_{\mathcal{L}})_{i}$, respectively, as
\begin{align}
       \boldsymbol{s}_{\mathcal{W}}= \boldsymbol{p}_{\mathcal{W}}\odot \boldsymbol{c}_{\mathcal{W}}^{\complement},
\end{align}
and
\begin{align}
   \boldsymbol{s}_{\mathcal{L}} = \boldsymbol{p}_{\mathcal{L}}\odot\boldsymbol{c}_{\mathcal{L}}^{\complement}.
\end{align}
Consequently, the average duration to support one successful transmission in the
unlicensed band can be calculated as
$
\boldsymbol{p}_{\mathcal{T}}^{\transpose}\boldsymbol{t}
$
where $\boldsymbol{p}_{\mathcal{T}}$ is defined in Table \ref{tbl:probs} and $\boldsymbol{t} = (T_{\text{idle}},~T_{s,\mathcal{W}},~T_{s,\mathcal{L}},~T_{c,\mathcal{W}},~T_{c,\mathcal{L}},~T_{c,\mathcal{W},\mathcal{L}})^{\transpose}\in \mathbb{R}^6$. For the chosen communications protocols, $T_{s,\mathcal{L}}$, $T_{s,\mathcal{W}}$, $T_{c,\mathcal{W}}$, $T_{c,\mathcal{L}}$, and $T_{c,\mathcal{W},\mathcal{L}}$ indicate the average time that the channel is sensed occupied by an LAA successful transmission, a Wi-Fi successful transmission, a collision among the Wi-Fi transmissions, a collision among the LAA transmissions, and a collision between the Wi-Fi and the LAA transmissions, respectively. $T_{\text{idle}}$ is the duration of an empty slot time. The vector $\boldsymbol{t}$ is dictated by the given access mechanism. Here, we consider the basic access mechanism as in \cite{Bianchi-2000,Yao-2019}. Therefore, $\boldsymbol{t}$ is calculated as in \cite{Mosleh-VTC2020}.

\subsection{Model Computational Details}
In order to improve the computational speed of the optimization routine, we rewrite some model details into more efficient forms. Specifically, we can write the LAA and Wi-Fi overall probability of transmission as
$
1 - \det\left( \text{diag}(\boldsymbol{p}_{\mathcal{L}}^{\complement})\right)
$
and
$
1 - \det\left( \text{diag}(\boldsymbol{p}_{\mathcal{W}}^{\complement})\right)
$
respectively, where
$$
\det\left( \text{diag}(\boldsymbol{p}_{\mathcal{K}}^{\complement})\right) = \prod_{k\in \mathcal{K}}(1 - \boldsymbol{e}_k^\transpose\boldsymbol{p}_{\mathcal{K}})
$$
such that $\boldsymbol{e}_k$ is the $k$-th column of the appropriately sized identity matrix for either network and $\mathcal{K}$ is a placeholder for either $\mathcal{L}$ or $\mathcal{W}$. Note that, $\boldsymbol{p}_{\mathcal{L}}$ and $\boldsymbol{p}_{\mathcal{W}}$ each depend on all probabilities and parameters given by the simultaneous non-linear system of four vector-valued equations, $\boldsymbol{p}_{\mathcal{W}}, \boldsymbol{c}_{\mathcal{W}} \in [0,1]^{W}$ and $\boldsymbol{p}_{\mathcal{L}}, \boldsymbol{c}_{\mathcal{L}} \in [0,1]^{L}$, for a total of $2(W + L)$ equations and unknowns: $\boldsymbol{p}_{\mathcal{L}}, \boldsymbol{p}_{\mathcal{W}}, \boldsymbol{c}_{\mathcal{L}}, \boldsymbol{c}_{\mathcal{W}}$. We solve the non-linear system using Levenberg-Marquardt to admit a set of consistent Wi-Fi AP and LAA eNodeB probabilities of transmission and collision for given parameters $\boldsymbol{\omega}_{\mathcal{W}}, \boldsymbol{\mu}_{\mathcal{W}} \in \mathbb{R}^{W}$ and $\boldsymbol{\omega}_{\mathcal{L}}, \boldsymbol{\mu}_{\mathcal{L}} \in \mathbb{R}^L$.

\subsection{Physical Layer Parameters and Data Rates}
In order to calculate the network throughput, we also need to introduce data rates and associated physical layer parameters. The achievable physical data rate of the $\mathcal{K}$-th operator is a function of link signal-to-noise ratio (SNR) which depends on changes with the link distances and propagation model. The link distances and propagation model admit parameter dependencies which are quantified in the subset of PHY layer parameters in $\boldsymbol{\theta}$. The subsequent data rate dependencies are expressed as $\log_{2}(1+\text{SNR}_{\mathcal{K}}(\boldsymbol{\theta}; \boldsymbol{x}))$
%\begin{align}
 %   \delta r_{\mathcal{K}}(\boldsymbol{\theta}; \boldsymbol{x}) &= 
%\end{align}
where $\boldsymbol{\theta}$ and $ \boldsymbol{x}$ are vectors representing the full set of parameters which can be varied to study the model behavior and the remaining \emph{fixed} scenario parameters, respectively. These parameter sets are discussed in detail in the following sub-section.

\subsection{Parametrized Model}
We parametrize MAC layer parameters by assuming common minimum contention window sizes and maximum back-off stages for each network. In other words, $\boldsymbol{\omega}_{\mathcal{W}} = \theta_1\boldsymbol{1}_{\mathcal{W}}$, $\boldsymbol{\omega}_{\mathcal{L}} = \theta_2\boldsymbol{1}_{\mathcal{L}}$, $\boldsymbol{\mu}_{\mathcal{W}} = \theta_3\boldsymbol{1}_{\mathcal{W}}$, and $\boldsymbol{\mu}_{\mathcal{L}} = \theta_4\boldsymbol{1}_{\mathcal{L}}$ for parameters $\theta_k \in \mathbb{R}$. Consequently, the minimum contention window sizes and maximum back-off stages are common across a particular network. It is conceivable that we may consider each independently for a total of $2(L + W)$ parameters as entries in a vector $\boldsymbol{\theta}$. However, we opt for a simplification to four total parameters---two common parameters per network. These parametrizations result in subsequent dependencies. Thus, in general, we consider $\boldsymbol{\mu}_{\mathcal{K}}(\boldsymbol{\theta})$ and $\boldsymbol{\omega}_{\mathcal{K}}(\boldsymbol{\theta})$ where $\mathcal{K}$ is either $\mathcal{W}$ or $\mathcal{L}$ and $\boldsymbol{\theta}$ is a vector of all parameters. Notice that certain partial derivatives are zero in this general vector-valued map interpretation, e.g., $\partial (\boldsymbol{\omega}_{\mathcal{W}})_j /\partial (\boldsymbol{\theta})_k =0$ for all $k=2,\dots,4$ and $j=1,\dots,W$. This may suggest some degeneracy in computations of the Jacobians which subsequently inform gradients of KPIs via the chain rule. Hence, certain directions in the parameter space may be more or less informative in changing various KPI predicted by this model. Regardless, we can now reinterpret the various probabilities as dependent maps $\boldsymbol{p}_{\mathcal{K}}(\boldsymbol{\theta})$ and $\boldsymbol{c}_{\mathcal{K}}(\boldsymbol{\theta})$ for either network $\mathcal{K}$ which depend on variations in $\boldsymbol{\theta}$. Notice any change in the input parameters $\boldsymbol{\theta}$ requires a new solution to the non-linear system. These subsequent solves dominate the computational expense of the model given new parameters $\boldsymbol{\theta}$.

We also append the physical parameters to the MAC parameter vector by reassigning $\boldsymbol{\theta}$ as a vector representing the full set of parameters which can be varied to study the model behavior. These additional PHY parameters are summarized with appropriate bounds and description as the remaining entries of $\boldsymbol{\theta}$ in Table \ref{Tb1}. Any remaining physical parameters are held fixed and constitute a \textit{scenario} for a particular model evaluation. We aggregate these remaining scenario parameters into a vector $\boldsymbol{x}$, summarized in Table \ref{Tb1}.

The LAA and Wi-Fi throughputs, indicated respectively by $f_{\mathcal{L}}$ and $f_{\mathcal{W}}$, are functions of $D$ total MAC and PHY layer parameters in a vector $\boldsymbol{\theta}$ conditioned on fixed values in a vector $\boldsymbol{x}$,
\begin{align} \label{eq:throughputs}
f_{\mathcal{L}}&: \mathbb{R}^D \times \lbrace \boldsymbol{x} \rbrace \rightarrow \mathbb{R}:(\boldsymbol{\theta}, \boldsymbol{x}) \mapsto f_{\mathcal{L}}(\boldsymbol{\theta}; \boldsymbol{x}),\\ \nonumber
f_{\mathcal{W}}&: \mathbb{R}^D\times \lbrace \boldsymbol{x} \rbrace \rightarrow \mathbb{R}:(\boldsymbol{\theta}, \boldsymbol{x}) \mapsto f_{\mathcal{W}}(\boldsymbol{\theta}; \boldsymbol{x}).
\end{align}
which are computed as
\begin{equation}\label{eq:throughput_full}
     f_{\mathcal{K}}(\boldsymbol{\theta}; \boldsymbol{x}) = T_{\mathcal{K}}\log_{2}(1+\text{SNR}_{\mathcal{K}}(\boldsymbol{\theta}; \boldsymbol{x}))\frac{\boldsymbol{p}_{\mathcal{K}}^{\transpose}(\boldsymbol{\theta})\boldsymbol{c}^{\complement}_{\mathcal{K}}(\boldsymbol{\theta})}{\boldsymbol{t}^{\transpose}\boldsymbol{p}_{\mathcal{T}}(\boldsymbol{\theta})}
\end{equation}
for arbitrary $\mathcal{K}$ representing either $\mathcal{L}$ or $\mathcal{W}$, where  $T_{\mathcal{K}}$ indicates the $\mathcal{K}$-th operator payload duration. We note that the numerator in \eqref{eq:throughput_full} is simply the sum of successful probabilities, $\boldsymbol{1}_{\mathcal{K}}^\transpose\boldsymbol{s}_{\mathcal{K}}(\boldsymbol{\theta}),$
similarly for the second and third entries of $\boldsymbol{p}_{\mathcal{T}}(\boldsymbol{\theta})$. This facilitates an intuitive explanation that throughput is simply the proportion of successful transmissions to all remaining transmission events if data rates are held constant.

For this application, LAA throughput $f_{\mathcal{L}}$ and Wi-Fi throughput $f_{\mathcal{W}}$ are only considered functions of $D$ variable parameters in $\boldsymbol{\theta}$. This numerical study considers $D=17$ parameters summarized in Table \ref{Tb1}. To simplify this study, we fix the remaining parameters in $\boldsymbol{x}$ governing the majority of the physical characteristics of the communication network---constituting a fixed \emph{scenario} $\boldsymbol{x}$ for a parameter study over $\boldsymbol{\theta}$'s. 

\subsection{Problem Formulation}
The problem of interest is to maximize a convex combination of network throughputs for the fixed scenario $\boldsymbol{x}$ over the MAC and PHY parameters $\boldsymbol{\theta}$ in a multi-criteria optimization. We define the \emph{Pareto front} by the following optimization problem:
\begin{equation} \label{eq:multiopt}
    \underset{\boldsymbol{\theta} \in \mathcal{D}  \subset \mathbb{R}^D}{\text{maximize}} \,\,tf_{\mathcal{L}}(\boldsymbol{\theta}; \boldsymbol{x}) + (1-t)f_{\mathcal{W}}(\boldsymbol{\theta}; \boldsymbol{x}),
\end{equation}
for all $t \in [0,1]$ where $\mathcal{D}$ is the parameter domain defined by the ranges in Table \ref{Tb1}. We refer to $t=0$ and $t=1$ as \emph{left} and \emph{right} solutions, respectively. The goal is to quantify a smooth trajectory $\boldsymbol{\theta}(t)$ through MAC and PHY parameter space, or \emph{trace} \cite{bolten2020tracing}, such that the convex combination of throughputs is maximized over a map $\boldsymbol{\theta}:[0,1] \rightarrow \mathcal{D}$. In Section \ref{sec:pareto_tracing} we formalize this notion of a trace. In Section \ref{sec:AS}, we summarize an exploratory approach for understanding to what extent problem \eqref{eq:multiopt} is convex \cite{boyd2004convex} and how we can intuitively regularize given the possibility of degeneracy induced by the chosen parametrization or otherwise. The empirical evidence generated through visualization and dimension reduction provide justification for convex quadratic approximations and subsequent quadratic trace in Section \ref{sec:Numerics}. 



\begin{table*}[t]
\captionsetup{font=footnotesize}
 \caption{MAC and PHY parameters influencing throughputs }\label{Tb1}
 \begin{threeparttable}
 \centering
 \scalebox{0.98}{
 \scriptsize
  \begin{tabular}{c|p{3.4cm} |c|c}
    \hline
    Parameters & Description &Bounds & Nominal \\ \hline
    %\rowcolor{LightCyan}
     $(\boldsymbol{\theta})_1$ & Wi-Fi min contention window size&(8, 1024)& 516\\[0.1cm] %\hline
      %\rowcolor{LightCyan}
  $(\boldsymbol{\theta})_2$ &  LAA min contention window size&(8, 1024)& 516\\[0.1cm] %\hline
   %\rowcolor{LightCyan}
    $(\boldsymbol{\theta})_3$ & Wi-Fi max back-off stage &(0, 8)& 4\\[0.1cm] %\hline
     %\rowcolor{LightCyan}
    $(\boldsymbol{\theta})_4$ & LAA max back-off stage&(0, 8)& 4\\[0.1cm] %\hline
    %\rowcolor{LightCyan}
    $(\boldsymbol{\theta})_{5}$ & Distance between transmitters &(10 m, 20 m)& 15 m\\[0.1cm]
    %\rowcolor{LightCyan}
    $(\boldsymbol{\theta})_{6}$ & Minimum distance between transmitters and receivers&(10m, 35 m)& 22.5 m\\[0.1cm]
    %\rowcolor{LightCyan}
    $(\boldsymbol{\theta})_{7}$ & Height of each LAA eNodeB and Wi-Fi AP&(3 m, 6 m) & 4.5 m\\[0.1cm]
    %\rowcolor{LightCyan}
    $(\boldsymbol{\theta})_{8}$ & Height of each LAA UEs and Wi-Fi STAs & (1 m, 1.5 m) & 1.25 m\\[0.1cm]
        %\rowcolor{LightCyan}
    $(\boldsymbol{\theta})_9$ & Standard deviation of shadow fading& (8.03, 8.29) & 8.16 \\[0.1cm]
    %\rowcolor{LightCyan}
    $(\boldsymbol{\theta})_{10}$ & $k_{\text{LOS}}^{\star}$
    %LoS path-loss constant$^\star$
    & (45.12, 46.38)& 45.75\\[0.1cm]%$32.4+20\log_{10}(5)$& $83.5+20\log_{10}(5)$
    %\rowcolor{LightCyan}
    $(\boldsymbol{\theta})_{11}$ & $k_{\text{NLOS}}^{\star}$
    %Non-LoS path-loss constant$^\star$
    & (34.70, 46.38) & 40.54\\[0.1cm]%$17.3+24.9\log_{10}(5)$& $141.4+20\log_{10}(5)$
   %$x_{12}$ & standard deviation of  &--&--\\[0.1cm]
  \end{tabular} \hspace{0.12in}
  \begin{tabular}{c|p{3.4cm} |c|c}
    \hline
    Parameters & Description &Bounds & Nominal \\ \hline
    %\rowcolor{LightCyan}
    $(\boldsymbol{\theta})_{12}$ &  $\alpha_{\text{LoS}}^{\star}$ 
    %LoS path-loss exponent$^\star$
    & (17.3, 21.5) & 19.4 \\[0.1cm]%The LoS path-loss exponent at each network
    %\rowcolor{LightCyan}
    $(\boldsymbol{\theta})_{13}$ &  $\alpha_{\text{NLoS}}^{\star}$
    %Non-LoS path-loss exponent$^\star$ 
    &(31.9, 38.3) & 35.1\\[0.1cm] %The NLoS path-loss exponent at each network 
    %\rowcolor{LightCyan}
    $(\boldsymbol{\theta})_{14}$ & Antenna gain at each transmitter &(0 dBi, 5 dBi) & 2.5 dBi\\[0.1cm]
    %\rowcolor{LightCyan}
    $(\boldsymbol{\theta})_{15}$ & Noise figure at each receiver&(5 dB, 9 dB) & 7 dB\\[0.1cm]
        %\rowcolor{LightCyan}
    $(\boldsymbol{\theta})_{16}$ & Transmit power at each LAA eNodeB and Wi-Fi AP&(18 dBm, 23 dBm) & 20.5 dBm\\[0.1cm]
    %\rowcolor{LightCyan}
    $(\boldsymbol{\theta})_{17}$ & Carrier channel bandwidth &(10 MHz, 20 MHz) & 15 MHz\\ [0.1cm]
    \rowcolor{Gray}
    $(\boldsymbol{x})_1$ & Number of LAA eNodeBs ($L$) &--& 6\\[0.1cm] %\hline
    \rowcolor{Gray}
    $(\boldsymbol{x})_2$ & Number of Wi-Fi APs ($W$) &--& 6\\[0.1cm] %\hline
    \rowcolor{Gray}
    $(\boldsymbol{x})_3$ & Number of LAA UEs &--& 6\\[0.1cm] %\hline
    \rowcolor{Gray}
    $(\boldsymbol{x})_4$ & Number of Wi-Fi STAs &--&6\\[0.1cm] %\hline
    \rowcolor{Gray}
    $(\boldsymbol{x})_5$ & Number of unlicensed channels &--& 1\\[0.1cm] %\hline
    %$(\boldsymbol{x})_6$ & Ideal slot time for LTE-LAA &--&--\\[0.1cm]
    \rowcolor{Gray}
    $(\boldsymbol{x})_{8}$ &  Scenario width &--&120 m\\[0.1cm]
    \rowcolor{Gray}
    $(\boldsymbol{x})_{9}$ &  Scenario height &--&80 m
    \end{tabular}}
     \begin{tablenotes}
           \item \text{Note: parameter ranges are established by 3GPP TS 36.213 V15.6.0 and 3GPP TR. 36.889 v13.0.0.}
      \item  \text{${}^{\star}$The path-loss for both line-of-sight (LoS) and non-LoS scenarios can be computed as $k + \alpha\log_{10}(d)$ in dB, where $d$ is the distance in meters }
      \item \text{between the transmitter and the receiver.}
    \end{tablenotes}
   \end{threeparttable}
\end{table*}
\normalsize
